Hegedus' Conjecture and Tighter Upper Bounds for Equidistant Codes in Hamming Spaces

An equidistant code is a code in the Hamming space such that two distinct codewords have the same Hamming distance. This paper investigates the bounds for equidistant codes in Hamming spaces.

==> draft.tex <==
\subsection{Improvement of Deza's theorem}

Let $X$ be a finite set of cardinality $n$. If $L = \{l_1,\ldots, l_r\}$ is a set of non negative integers with $l_1 < l_2 < \cdots< l_r$, and $k$ is a natural number, then by an $(n,k,L)$-system we mean a collection of $k$-element subsets of $X$ such that the intersection of any two different sets has cardinality belonging to $L$. 

A family $\mathcal{F} = \{B_1, B_2,\ldots, B_m\}$ of sets is called a $\Delta$-system of cardinality $m$ if there exists a set $D \subseteq B_i$, with $i = 1,\ldots,m$, such that the sets $B_1\backslash D,\cdots,B_m\backslash D$ are pairwise disjoint. $D$ is called the kernel of the $\Delta$-system.

\begin{theorem}[Deza\cite{Deza1974},1976]
\label{Theorem_deza_Delta_system}
    An $(n, k,l)$-system $\mathcal{F}$ of cardinality more than
 $k^2-k+1$ is a $\Delta$-system and thus
 \[|\mathcal{F}|\le \frac{n-l}{k-l}.\]
\end{theorem}

The following example shows that this result is tight when $l = 1$.

\begin{example}
\label{example_finite_projective_plane}
    A finite projective plane of order $q$ is a $2-(q^2+q+1,q+1,1)$ design, namely, any two points determine a unique line and any two line intersect in a unique point. Let $\mathcal{D}$ be a finite projective plane of order $q$. Then $\mathcal{D}$ has $q^2+q+1$ lines. Therefore it is an $(n = q^2+q+1,k = q+1,l = 1)$-system of cardinality $m = q^2+q+1$. It is clearly not a $\Delta$-system while satisfying that $m = k^2-k+1$.

\end{example}

Before applying Deza's theorem to simplex code, we shall investigate to what extent we can relax the condition required for the cardinality of the system in it.


\begin{proposition}
\label{proposition_(n,4,2)_system}
    An $(n,4,2)$-system $\mathcal{F}$ of cardinality $m> 7$ is a $\Delta$-system.
\end{proposition}

\begin{proof}
    Since $\mathcal{F}$ can be viewed as a binary simplex code, $m\le n+1$ and thus $n\ge 10$. Suppose $X$ with $|X|=n$ is the ground set of the family $\mathcal{F}$. For $x\in X$, we define the degree of it by
    \[\mathrm{deg}(x) = \#\{S\in \mathcal{F}:x\in F\}.\]
    We arrange the elements in $X$ such that 
    \[{\deg(x_1)\ge \deg(x_2)\ge \cdots\ge \deg(x_n)}.\]

    \textbf{Claim.} It must hold that $\deg(x_2)\ge 4$.
    
    Assume for contradiction that $\deg(x_2)\le 3$. Let $A \in\mathcal{F}$ and $\mathcal{F}' = \mathcal{F}\backslash\{A\}$. Denote $N_A$ the cardinality of the following set
    \[\{(a,S)\in A\times \mathcal{F}':a\in S\}.\]
     On one hand, $N_A = 2(m-1)$. On the other hand, 
     \[N_A = \sum_{a\in A}(\deg(x)-1)=\sum_{a\in A}\deg(x)-4.\]
     Thus $N_A\le \deg(x_1)+\deg(x_2)+\deg(x_3)+\deg(x_4)-4\le m+3+3+3-4 = m+5$. Therefore, $2(m-1)\le m+5$, which implies $m\le 7$, a contradiction.

     Now we have $\deg(x_1)\ge \deg(x_2)\ge 4$. Suppose $x_1,x_2$ are contained in $A_1,A_2,A_3,A_4\in \mathcal{F}$. For any $S\in \mathcal{F}$ not equal to $A_i$ with $i\in[4]$, in order to intersect each $A_i$ in exactly two elements, $S$ must contain $x_1,x_2$, which finishes the proof.
\end{proof}

Note that this result is tight in the sense that there exists a $(7,4,2)$-system of cardinality $7$ which is not a $\Delta$-system.

\begin{example}
\label{example_system_from_Hadamard_code}
    Consider the simplex code given in Example \ref{example_simplex_code_maximum_size} for $q=2$, which is a $[7,3,4]_2$ linear simplex code of cardinality $8$, denoted by $C$. The set of all nonzero codewords in $C$ actually forms a $(7,4,2)$-system of cardinality $7$, and it is not a $\Delta$-system.
\end{example}

\begin{remark}
    The idea of considering the degree of the elements come from the work of Deza, Erd\"{o}s and Frankl in \cite{DezaErdosFrankl1978}. We can push forward this idea to strengthen Theorem \ref{Theorem_deza_Delta_system} whenever $l\ge 1$.
\end{remark}


Formally, we define the degree of $x\in X$ in family $\mathcal{F}$ to be
\[\deg_\mathcal{F}(x) = \#\{S\in \mathcal{F}:x\in \mathcal{F}\}\]
and the degree of a subsets $A\subseteq X$ to be
\[\deg_{\mathcal{F}}(A)=\sum_{x\in X}\deg_\mathcal{F}(x).\]

\begin{lemma}
\label{lemma_summation_of_degree}
    Let $\mathcal{F}\subseteq 2^X$ be an $(n,k,l)$-system of cardinality $m$. Let $A\in \mathcal{F}$ and $\mathcal{F'} = \mathcal{F}\backslash\{A\}$. Then we have the following results.
    \begin{enumerate}
        \item[(a)] $\deg_\mathcal{F}(X) =km$;
        \item[(b)] $\deg_{\mathcal{F'}}(A) =l(m-1)$;
        \item[(c)] $\deg_\mathcal{F'}(A)=\deg_\mathcal{F}(A)-k$.
    \end{enumerate}
\end{lemma}

\begin{proof}
    The claim (a) follows by double counting the set
    \[\{(x,S)\in X\times \mathcal{F}:x\in S\}.\]

    The claim (b) follows by double counting the set
    \[\{(x,S)\in A\times \mathcal{F'}:x\in S\}.\]

    To prove the claim (c), we observe that for all $x\in A$, $\deg_\mathcal{F'}(x) = \deg_\mathcal{F}(x)-1$, thus 
    \[\deg_{\mathcal{F'}}(A) = \sum_{x\in A}\deg_{\mathcal{F'}}(x) = \sum_{x\in A}(\deg_{\mathcal{F}}(x)-1) = \deg_{\mathcal{F}}(A)-k,\]
    which completes the proof.
\end{proof}


\begin{theorem}
     An $(n,k,l)$-system $\mathcal{F}\subseteq 2^X$ of cardinality $m> (k-l+1)^2-k+l$ is a $\Delta$-system.
\end{theorem}

\begin{proof}
    Let $t = k-l+1$. We arrange the elements in $X$ such that
    \[{\deg_\mathcal{F}(x_1)\ge \deg_\mathcal{F}(x_2)\ge \cdots\ge \deg_\mathcal{F}(x_n)}.\]

   We claim that $\deg_\mathcal{F}(x_{l})\ge t+1$. Assume for contradiction that $\deg(x_l)\le t$. Let $A \in\mathcal{F}$ and $\mathcal{F}' = \mathcal{F}\backslash\{A\}$. Then by Lemma \ref{lemma_summation_of_degree} (b) we have
    \[\deg_\mathcal{F'}(A)=l(m-1).\]
    Meanwhile by Lemma \ref{lemma_summation_of_degree} (c) 
    \begin{align*}
       \deg_\mathcal{F'}(A)& = \deg_{\mathcal{F}}(A)-k\le \sum_{i = 1}^{k}\deg_\mathcal{F}(x_i)-k\\
        &\le (l-1)m+(k-l+1)t-k= (l-1)m+t^2-k.
    \end{align*}
    Therefore, we have $l(m-1)\le  (l-1)m+t^2-k$, thus $m\le t^2-k+l$, which contradicts that $m> t^2-k+l$.
    
    Now we have $\deg_\mathcal{F}(x_1)\ge \cdots \ge \deg_\mathcal{F}(x_l)\ge t+1$. Assume $x_1,x_2,\ldots,x_l$ are contained in $A_1,A_2,\ldots, A_{t+1}\in \mathcal{F}$. Denote $\mathcal{F''} = \{A_1,A_2,\ldots,A_{t+1}\}$. For any $S\in \mathcal{F}\backslash\mathcal{F''}$, suppose 
    \[\#\{x_i:i\in [l], x_i\in S\} = r.\]
    By Lemma \ref{lemma_summation_of_degree} (b) we have $\deg_{\mathcal{F''}}(S) = (t+1)l$. On the other hand, 
    \[\deg_{\mathcal{F''}}(S) = \sum_{x\in S}\deg_{\mathcal{F''}}(x) \le r(t+1)+(k-r). \]
    Therefore, $(t+1)l\le r(t+1)+k-r$ and thus 
    \[(k-l+1)(l-r)\le k-l,\]
    which only holds for $r = l$, namely, $S$ contains all $x_i$ for $i = 1,2,\ldots,l$. The proof is now complete.
     
\end{proof}

\begin{problem}
    For general positive integer $l$, what is the smallest $m_0(k,l)$ such that any $(n,k,l)$-system with cardinality $m>m_0(k,l)$ is a $\Delta$-system?
\end{problem}

We know that \( m_0(k,1) = k^2 - k + 1 \) follows from Deza's Theorem \ref{Theorem_deza_Delta_system} and Example \ref{example_finite_projective_plane}. Similarly, Proposition \ref{proposition_(n,4,2)_system} and Example \ref{example_system_from_Hadamard_code} establish that \( m_0(4,2) = 7 \).

\begin{corollary}
\label{corollary_system_for_simplex_code}
    An $(n,d,d/2)$-system $\mathcal{F}$ of cardinality $m> (d^2+2d+4)/4$ is a $\Delta$-system, where $d$ is an even positive integer.\hfill\qed
\end{corollary}

\subsection{Simplex codes in $H_q^n$}

We can reduce the \( q \)-ary case to the binary case to obtain an upper bound on the size of $q$-ary simplex codes.

\begin{proposition}  
Let \( C \subseteq H_q^n \) be a simplex code with distance \( d \). If \( n \geq \frac{2d(2d^2 - d + 1)}{q} \), then  
\[
|C| \leq \frac{q n}{d}.
\]
\end{proposition}

\begin{proof}
For \( i = 0, 1, \ldots, q-1 \), let \( e_i \in H_2^q \) be the vector with a one in the \( (i+1) \)-th coordinate and zeros elsewhere. Define the mapping  
\[
\rho: C \rightarrow H_2^{q n}, \quad [a_1 \, a_2 \, \cdots \, a_n] \mapsto [e_{a_1} \, e_{a_2} \, \cdots \, e_{a_n}].
\]  
This mapping \( \rho \) transforms the \( q \)-ary simplex code \( C \) with distance \( d \) into a binary simplex code \( \rho(C) \subseteq H_2^{q n} \) with distance \( 2d \). By Proposition \ref{proposition_upper_bound_with_d_binary_case} (b), if  
\[
q n \geq \frac{2d \left( (2d)^2 - 2d + 2 \right)}{2} = 2d(2d^2 - d + 1),
\]  
then  
\[
|C| \leq \frac{2 q n}{2 d} = \frac{q n}{d}.
\]
\end{proof}

In this approach, we use the standard basis vectors \( \{e_0, e_1, \ldots, e_{q-1}\} \) to encode the \( q \)-ary alphabet, thereby reducing the \( q \)-ary case to the binary case. However, employing a more carefully designed binary simplex code could potentially yield a sharper bound. 

For a positive integer $k$, there exists a binary simplex code $\mathcal{A}_{2^k} \subseteq H_2^{2^k - 1}$ with length $2^k - 1$, cardinality $2^k$, and distance $2^{k-1}$. Let $q = 2^k$ and $\mathcal{A}_q = \{v_0, v_1, \ldots, v_{q-1}\} \subseteq H_2^{q-1}$, where $v_0 = 0$. Define the mapping
\[
\varphi_k: H_q^n \to H_2^{(q-1)n}, \quad a = [a(1)\ a(2)\ \ldots\ a(n)] \mapsto [v_{a(1)}\ v_{a(2)}\ \ldots\ v_{a(n)}],
\]
where $\varphi_k$ preserves distances and weights up to scaling: $\mathrm{wt}(\varphi_k(x)) = 2^{k-1} \cdot \mathrm{wt}(x)$ and $\mathrm{d_H}(\varphi_k(x), \varphi_k(y)) = 2^{k-1} \cdot \mathrm{d_H}(x, y)$.

\begin{theorem}
\label{theorem_upper_bound_with_d_in_case_q=2^k}
    Let $q = 2^k$ for some positive integer $k$, and let $C \subseteq H_q^n$ be a simplex code with distance $d$. If
    \[
    n \geq \frac{q d (q^2 d^2 - 2 q d + 8)}{16 (q - 1)},
    \]
    then
    \[
    |C| \leq \frac{4 (q - 1) n}{q d}.
    \]
\end{theorem}

\begin{proof}
    The code $\varphi_k(C) \subseteq H_2^{(q-1)n}$ is a binary simplex code with distance $2^{k-1} d = q d / 2$. Apply Proposition \ref{proposition_upper_bound_with_d_binary_case} to $\varphi_k(C)$ with length $(q-1)n$ and distance $qd/2$, we require:
    \[(q-1)n\ge \frac{qd/2[(qd/2)^2-(qd/2)+2]}{2},\]
    which simplifies to $n\ge \frac{qd(q^2d^2-2qd+8)}{16(q-1)}$. Therefore, with the given condition on $n$, we obtain
    \[
    |C| = |\varphi_k(C)| \leq \left\lfloor \frac{2 (q - 1) n}{q d / 2} \right\rfloor \le\frac{4 (q - 1) n}{q d}.
    \]
\end{proof}

\begin{theorem}
    Let $C \subseteq H_q^n$ be a simplex code with distance $d$. If
    \[
    n \geq  \frac{qd(q^2d^2-qd+2)}{2(2q-1)},
    \]
    then
    \[
    |C| \leq \frac{4 (2 q - 3) n}{(2 q - 2) d}.
    \]
\end{theorem}

\begin{proof}
    Assume $2^{k-1} + 1 \leq q \leq 2^k$. View $C \subseteq H_{2^k}^n$. By Theorem \ref{theorem_upper_bound_with_d_in_case_q=2^k},
    \begin{align*}
        |C| &\leq \frac{4 (2^k - 1) n}{2^kd} \le \frac{4 (2 q - 3) n}{(2 q - 2) d}, & \text{as } 2^k\le 2q-2
    \end{align*}
    provided 
    \begin{align*}
        n &\ge \frac{qd(q^2d^2-qd+2)}{2(2q-1)}&\text{by given condition}\\
         &= \frac{2qd[(2q)^2d^2-2(2q)d+8]}{16(2q-1)} \\
        &\geq \frac{2^k d [(2^k)^2 d^2 - 2\cdot2^k d + 8]}{16 (2^k - 1)} &\text{as }2q>2^k.
    \end{align*}
     
\end{proof}


These bounds suggest that for sufficiently large \( n \), the size of a \( q \)-ary simplex code is at most approximately \( \frac{4n}{d} \), with the alphabet size \( q \) exerting only a minor influence on this upper bound. In Theorem \ref{theorem_q_ary_case_bound_without_q}, we will prove a stronger result: when \( n \) is sufficiently large relative to both \( q \) and \( d \), the optimal construction of a \( q \)-ary simplex code closely resembles that of the binary case. To proceed, we first establish some preliminary concepts.

Henceforth, a binary word \( x \in H_2^n \) will be identified with its support subset \( \mathrm{supp}(x) \subseteq [n] \). For instance, if \( A \subseteq [n] \), then \( A \subseteq x \) means \( A \subseteq \mathrm{supp}(x) \), and for \( y \in H_2^n \), the intersection size \( |x \cap y| \) is defined as \( |\mathrm{supp}(x) \cap \mathrm{supp}(y)| \).

For a subset \( S \subseteq [n] \), we define a projection map that maps a subset \( A \subseteq [n] \) to its intersection with \( S \):
\[
\pi_S: 2^{[n]} \to 2^S, \quad A \mapsto A \cap S.
\]
This projection extends naturally to the binary Hamming space:
\[
\pi_S: H_2^{[n]} \to H_2^S, \quad x = [x(i) : i \in [n]] \mapsto [x(i) : i \in S],
\]
where \( H_2^n \) and \( H_2^S \) represent binary words indexed by \( [n] \) and \( S \), respectively.

\begin{lemma}
\label{lemma_projection_of_Delta_system}
Suppose \( \mathcal{F} \) is a \( \Delta \)-system with kernel \( D \). Then, for any subset \( S \subseteq [n] \), the projection \( \pi_S(\mathcal{F}) \) is also a \( \Delta \)-system with kernel \( \pi_S(D) \).
\end{lemma}

\begin{proof}
Let \( D \subseteq [n] \) be the kernel of the \( \Delta \)-system \( \mathcal{F} \). For any \( A \in \mathcal{F} \), since \( D \subseteq A \), we have \( \pi_S(D) = D \cap S \subseteq A \cap S = \pi_S(A) \). Furthermore, for any two distinct elements \( A_1, A_2 \in \mathcal{F} \), their intersection equals the kernel: \( A_1 \cap A_2 = D \). Thus,
\[
\pi_S(A_1) \cap \pi_S(A_2) = (A_1 \cap S) \cap (A_2 \cap S) = (A_1 \cap A_2) \cap S = D \cap S = \pi_S(D).
\]
This shows that \( \pi_S(\mathcal{F}) \) is a \( \Delta \)-system with kernel \( \pi_S(D) \). \hfill \(\qed\)
\end{proof}

\begin{remark}
The kernel \( \pi_S(D) \) of \( \pi_S(\mathcal{F}) \) may be empty. Additionally, distinct elements \( A_i \in \mathcal{F} \) may project to \( \pi_S(D) \), yielding identical images. Both cases are consistent with the definition of a \( \Delta \)-system.
\end{remark}

To establish our main result, we reduce a \( q \)-ary code to a binary code. Unlike previous methods, we avoid using a complex binary simplex code \( \mathcal{A}_q \) to encode the alphabet \( [0, q-1] \). Instead, define \( w_0 = \emptyset \) and \( w_i = \{i, q\} \) for \( i = 1, 2, \ldots, q-1 \). The set \( \mathcal{Q}_q = \{w_0, w_1, \ldots, w_{q-1}\} \), when viewed as a code in \( H_2^q \), forms a simplex code with distance 2 and satisfies:
\begin{enumerate}
    \item \( w_i \neq \emptyset \) if and only if \( i \neq 0 \),
    \item \( |w_i \cap w_j| = \begin{cases} 
    0, & \text{if } i = 0 \text{ or } j = 0, \\ 
    1, & \text{if } i, j \neq 0 \text{ and } i \neq j, \\ 
    2, & \text{if } i = j \neq 0.
    \end{cases} \)
\end{enumerate}

These properties lead directly to the following lemma.

\begin{lemma}
\label{lemma_Delta_system_of_Q_q}
Let \( x_1, x_2, \ldots, x_m \) be elements chosen from \( \mathcal{Q}_q \), possibly with repetition. If \( |x_i \cap x_j| = 1 \) for all \( i \neq j \), then all \( x_i \) are nonzero and distinct in \( \mathcal{Q}_q \), implying \( m \leq q-1 \). \hfill \(\qed\)
\end{lemma}

Define the mapping:
\[
\psi: H_q^n \to H_2^{q n}, \quad a = [a(1) \, a(2) \, \cdots \, a(n)] \mapsto [w_{a(1)} \, w_{a(2)} \, \cdots \, w_{a(n)}].
\]
Like \( \varphi_k \), the map \( \psi \) scales weight and distance: \( \mathrm{wt}(\psi(x)) = 2 \cdot \mathrm{wt}(x) \) and \( \mathrm{d_H}(\psi(x), \psi(y)) = 2 \cdot \mathrm{d_H}(x, y) \). By replacing each symbol in \( [0, q-1] \) with a \( q \)-length vector, \( \psi \) induces a partition of the coordinate set \( [q n] \):
\[
[q n] = \bigcup_{i=1}^n I_i, 
\]
where $I_i := [q(i-1)+1, q i]$ for $i = 1, 2, \ldots, n$.

\begin{definition}
A code \( C \subseteq H_q^n \) of constant weight \( k \) is a \textbf{\( \Delta_q(n, k, l) \)-system} with kernel \( D \subseteq [n] \), where \( |D| = l \), if for any two distinct codewords \( x, y \in C \):
\begin{enumerate}
    \item \( x(i) = y(i) \neq 0 \) for all \( i \in D \),
    \item \( x(i) = 0 \) or \( y(i) = 0 \) for all \( i \in [n] \backslash D \).
\end{enumerate}
For \( q = 2 \), a \( \Delta_2(n, k, l) \)-system corresponds to a \( \Delta(n, k, l) \)-system via the support set of each codeword, allowing us to drop the subscript and call it a \( \Delta(n, k, l) \)-system.
\end{definition}

\begin{theorem}
\label{theorem_q_ary_case_bound_without_q}
Let \( C \subseteq H_q^n \) be a simplex code with distance \( d \), containing the all-zero codeword.
\begin{itemize}
    \item[(a)] If \( |C| > \max\{4 d^2 - 2 d + 2, q\} \), then \( d \) is even, and \( C \backslash \{0\} \) is a \( \Delta_q(n, d, d/2) \)-system, so:
    \[
    |C| \leq \left\lfloor \frac{2 n}{d} \right\rfloor.
    \]
    \item[(b)] If \( n \geq \max\{2 d^3 - 2 d^2 + d, \frac{q d}{2}\} \), then:
    \[
    |C| \leq \left\lfloor \frac{2 n}{d} \right\rfloor.
    \]
\end{itemize}
\end{theorem}

\begin{proof}
We utilize the map \( \psi \) and the partition \( \{I_i : i \in [n]\} \) of \( [q n] \) defined earlier.

Since \( C \) includes the all-zero vector, all codewords in \( C' = C \backslash \{0\} \) have weight \( d \). Applying \( \psi \) to \( C \) produces a simplex code \( \psi(C) \subseteq H_2^{q n} \) with distance \( 2d \). As \( \psi(C) \) contains the all-zero codeword and \( \psi(C') \) has constant weight \( 2d \), \( \psi(C') \) forms an \( (q n, 2d, d) \)-family. If \( |C| > 4 d^2 - 2 d + 2 \), then \( |\psi(C')| = |C'| > (2d)^2 - 2d + 1 \), and by Theorem \ref{Theorem_deza_Delta_system}, \( \psi(C') \) is a \( \Delta(q n, 2d, d) \)-system with kernel \( D \subseteq [q n] \) of size \( |D| = d \).

Consider the projection of \( \psi(C') \) onto \( I_i \) for each \( i \in [n] \):
\[
\pi_{I_i}(\psi(C')) = \{\pi_{I_i}([w_{a(1)} \, w_{a(2)} \, \cdots \, w_{a(n)}]) : a \in C'\} = \{w_{a(i)} : a \in C'\}.
\]
By Lemma \ref{lemma_projection_of_Delta_system}, \( \pi_{I_i}(\psi(C')) \) is a \( \Delta \)-system with kernel \( \pi_{I_i}(D) = D \cap I_i \). Since \( \psi(C') \) is a \( \Delta \)-system with kernel \( D \), for distinct \( x, y \in C' \),
\[
D = \psi(x) \cap \psi(y) = [w_{x(j)} \cap w_{y(j)} : j \in [n]\, ],
\]
so:
\[
|D \cap I_i| = |(\psi(x) \cap \psi(y)) \cap I_i| = |w_{x(i)} \cap w_{y(i)}|.
\]

We now prove that \( C' \) is a \( \Delta_q(n, d, d/2) \)-system with kernel:
\[
K = \{i \in [n] : I_i \cap D \neq \emptyset\}.
\]

\textbf{Step 1.} For \( i \in K \), show \( a(i) \neq 0 \) for all \( a \in C' \). Since \( I_i \cap D \neq \emptyset \) and \( I_i \cap D \subseteq w_{a(i)} \), we have \( w_{a(i)} \neq \emptyset \), implying \( a(i) \neq 0 \).

\textbf{Step 2.} For \( i \in K \), show \( x(i) = y(i) \) for any distinct \( x, y \in C' \). Assume there exist distinct \( a, b \in C' \) with \( a(i) \neq b(i) \). Since \( a(i), b(i) \neq 0 \) (by Step 1), \( |w_{a(i)} \cap w_{b(i)}| = 1 \). Thus, for any distinct \( x, y \in C' \),
\[
|w_{x(i)} \cap w_{y(i)}| = |D \cap I_i| = 1,
\]
and by Lemma \ref{lemma_Delta_system_of_Q_q}, \( |\{w_{x(i)} : x \in C'\}| = |C'| \leq q-1 \). However, \( |C'| > q \), a contradiction. Hence, \( x(i) = y(i) \).

\textbf{Step 3.} For \( i \in [n] \backslash K \), show that for distinct \( x, y \in C' \), either \( x(i) = 0 \) or \( y(i) = 0 \). Since \( D \cap I_i = \emptyset \), the kernel of \( \pi_{I_i}(\psi(C')) = \{w_{a(i)} : a \in C'\} \) is empty, so:
\[
|w_{x(i)} \cap w_{y(i)}| = |D \cap I_i| = 0,
\]
implying \( w_{x(i)} = \emptyset \) or \( w_{y(i)} = \emptyset \), i.e., \( x(i) = 0 \) or \( y(i) = 0 \).

These steps confirm that \( C' \) is a \( \Delta_q(n, d, |K|) \)-system. To find \( |K| \), note that for distinct \( x, y \in C' \), \( x(i) = y(i) \neq 0 \) for \( i \in K \) (Steps 1 and 2), so \( |w_{x(i)} \cap w_{y(i)}| = 2 \). Thus:
\[
D = \bigcup_{j=1}^n (D \cap I_j) = \bigcup_{j \in K} (D \cap I_j),
\]
\[
|D| = \sum_{j \in K} |D \cap I_j| = \sum_{j \in K} 2 = 2 |K|.
\]
Since \( |D| = d \), we have \( d = 2 |K| \), so \( d \) is even and \( |K| = d/2 \). This proves part (a). Part (b) follows from part (a). 
\end{proof}



\begin{example}
\label{example_simplex_code_maximum_size}
    Let \( q \) be a prime power and \( \mathbb{F}_q \) the finite field of order \( q \). Let \( k \) be a positive integer. Consider all \( \frac{q^k - 1}{q-1} \) one-dimensional vector subspaces in \( \mathbb{F}_q^k \). Choose one nonzero vector from each subspace, and define a matrix \( G \) with those chosen vectors as columns, say
    \[
    G = [v_1\ v_2\ \cdots\ v_{\frac{q^k - 1}{q-1}}].
    \]
    It can be verified that \( G \) generates an \( \left[ n = \frac{q^k - 1}{q-1}, k, d = q^{k-1} \right]_q \) simplex linear code \( C \). We show \( d = q^{k-1} \) below.

    For any nonzero codeword \( c \in C \), it can be written as
    \[
    c = x^T G = [\langle x, v_1 \rangle\ \langle x, v_2 \rangle\ \cdots\ \langle x, v_n \rangle],
    \]
    where \( x \) is some nonzero column vector in \( \mathbb{F}_q^k \) and \( \langle \cdot, \cdot \rangle \) represents the usual dot product. Note that \( x \) defines a hyperplane in \( \mathbb{F}_q^k \), that is,
    \[
    x^\perp = \{ y \in \mathbb{F}_q^k : \langle x, y \rangle = 0 \}.
    \]
    Since \( x^\perp \) is a \((k-1)\)-dimensional subspace containing \( q^{k-1} \) elements, it includes \( \frac{q^{k-1} - 1}{q-1} \) one-dimensional subspaces, each corresponding to one of the columns \( v_i \) in \( G \). Thus, the weight of \( c \) is
    \begin{align*}
        \mathrm{wt}(c) &= \#\{ i \in [n] : \langle x, v_i \rangle \neq 0 \} \\
        &= n - \#\{ i \in [n] : \langle x, v_i \rangle = 0 \} \\
        &= \frac{q^k - 1}{q-1} - \frac{q^{k-1} - 1}{q-1} \\
        &= q^{k-1},
    \end{align*}
    which implies that \( C \) is a constant weight code and thus a simplex code, with minimum distance \( d = q^{k-1} \).
    
    Note that \( d = q^{k-1} = \frac{n(q-1) + 1}{q} \), since \( n = \frac{q^k - 1}{q-1} \). Also, \( |C| = q^k = n(q-1) + 1 \). Thus, when \( d = \frac{n(q-1) + 1}{q} \), the bound \( |C| \leq n(q-1) + 1 \) is tight.% \hfill \(\qed\)
\end{example}


\subsection{Binary simplex codes}

Let $l \leq k\le n$ be non-negative integers. If $A \subseteq [n]$ has cardinality $k$, we call it a \textit{$k$-subset} of $[n]$. An \textit{$(n, k, l)$-family} is a collection of $k$-subsets of $[n]$ such that the intersection of any two distinct sets has cardinality exactly $l$.

A family $\mathcal{F} = \{B_1, B_2, \ldots, B_m\}$ of sets is called a \textit{$\Delta$-system} of cardinality $m$ if there exists a set $D \subseteq B_i$ for $i = 1, 2, \ldots, m$, such that the sets $B_1 \backslash D, B_2 \backslash D, \ldots, B_m \backslash D$ are pairwise disjoint. The set $D$ is referred to as the \textit{kernel} of the $\Delta$-system. A \textit{$\Delta(n, k, l)$-system} is a $\Delta$-system consisting of $k$-subsets of $[n]$ with a kernel of size $l$.

It is clear that a $\Delta(n, k, l)$-system is an $(n, k, l)$-family. The maximum cardinality of a $\Delta(n, k, l)$-system is given by
\[
\left\lfloor \frac{n - l}{k - l} \right\rfloor,
\]
since the $k - l$ elements in each $B_i \backslash D$ must be disjoint across all sets in the family, and there are $n - l$ elements available in $[n] \backslash D$. The following theorem demonstrates that this bound is optimal for sufficiently large $n$.

\begin{theorem}[Deza \cite{Deza1974}, 1976]
\label{Theorem_deza_Delta_system}
    An $(n, k, l)$-family $\mathcal{F}$ with cardinality greater than $k^2 - k + 1$ is a $\Delta(n,k,l)$-system, and thus
    \[
    |\mathcal{F}| \leq \frac{n - l}{k - l}.
    \]
\end{theorem}

The next example illustrates that the bound in Theorem \ref{Theorem_deza_Delta_system} is tight for $l = 1$, by exhibiting an $(n, k, 1)$-family with cardinality $k^2 - k + 1$ that is not a $\Delta$-system.

\begin{example}
\label{example_finite_projective_plane}
    A finite projective plane of order $q$ is a $2$-$(q^2 + q + 1, q + 1, 1)$ design, meaning that any two points determine a unique line, and any two lines intersect at exactly one point. It is known that such design exists when $q$ is a prime power. Let $\mathcal{D}$ be the set of lines in such a plane. Then $\mathcal{D}$ contains $q^2 + q + 1$ lines, each a $(q + 1)$-subset of a point set of size $n = q^2 + q + 1$. Thus, $\mathcal{D}$ is an $(n = q^2 + q + 1, k = q + 1, l = 1)$-family with cardinality $m = q^2 + q + 1$. Since $k = q + 1$, we have $m = k^2 - k + 1$, yet $\mathcal{D}$ is not a $\Delta$-system because no fixed kernel $D$ of size 1 can satisfy the pairwise disjointness condition.% \hfill \qed
\end{example}

For binary simplex codes, the distance $d$ plays a critical role. When $d$ is odd, a binary simplex code $C \subseteq H_2^n$ cannot contain more than two codewords. This follows because any two codewords of weight $d$ have an even Hamming distance, while a simplex code requires all pairwise distances to equal $d$. Thus, we focus on even $d$ henceforth.

\begin{example}
    We identify subsets of $[n]$ with their incidence vectors in $H_2^n$ when unambiguous. Let $n$ be a positive integer and $d$ an even positive integer. There exists a simplex code $C \subseteq H_2^n$ with distance $d$ and cardinality
    \[
    \left\lfloor \frac{2n}{d} \right\rfloor.
    \]
    
    One construction defines $C$ as a $\Delta(n, d/2, 0)$-system of size $\left\lfloor \frac{2n}{d} \right\rfloor$. Here, each codeword has weight $d/2$, and since the kernel is empty, all codewords are pairwise disjoint, yielding a Hamming distance of $d/2 + d/2 = d$. Thus, $C$ is a simplex code.

    Alternatively, let $D$ be a $\Delta(n, d, d/2)$-system of size
    \[
    \left\lfloor \frac{n - d/2}{d - d/2} \right\rfloor = \left\lfloor \frac{2n}{d} \right\rfloor - 1,
    \]
    and form $C = D \cup \{0\}$, where $0$ is the all-zero vector. Each codeword in $D$ has weight $d$, and the kernel of size $d/2$ ensures that any two distinct codewords in $D$ intersect in $d/2$ positions and differ in $d - d/2 = d/2$ positions outside the kernel, giving a distance of $d$. The distance from $0$ to any codeword in $D$ is $d$, so $C$ is a simplex code of size $\left\lfloor \frac{2n}{d} \right\rfloor$.

    Both constructions yield equivalent codes under translation. %\hfill $\qed$
\end{example}

\begin{proposition}
\label{proposition_upper_bound_with_d_binary_case}
    Let $C \subseteq H_2^n$ be a simplex code with even distance $d$.
    \begin{enumerate}
        \item[(a)] If $|C| > d^2 - d + 2$, then $C$ is equivalent to a $\Delta(n, d/2, 0)$-system, and thus
        \[
        |C| \leq \left\lfloor \frac{2n}{d} \right\rfloor.
        \]
        \item[(b)] If $n \geq \frac{d(d^2 - d + 2)}{2}$, then
        \[
        |C| \leq \left\lfloor \frac{2n}{d} \right\rfloor.
        \]
    \end{enumerate}
\end{proposition}

\begin{proof}
    Assume $C$ includes the all-zero codeword $0$. Then $C \backslash \{0\}$ is an $(n, d, d/2)$-family, as each codeword has weight $d$, and the distance $d$ implies an intersection of size $d/2$ between any two distinct codewords. If $|C|>d^2-d+2$, then $|C\backslash \{0\}| = |C|-1>d^2-d+1$. By Theorem \ref{Theorem_deza_Delta_system}, $C \backslash \{0\}$ is a $\Delta(n, d, d/2)$-system, and thus
    \[
    |C \backslash \{0\}| \leq \frac{n - d/2}{d - d/2} = \frac{2n}{d} - 1.
    \]
    Thus, $|C| \leq \left\lfloor \frac{2n}{d} \right\rfloor$, and $C$ is equivalent to a $\Delta(n, d/2, 0)$-system under translation. This proves (a).

    For (b), the bound $|C| \leq \max\{d^2 - d + 2, \left\lfloor \frac{2n}{d} \right\rfloor\}$ holds from (a). When $n \geq \frac{d(d^2 - d + 2)}{2}$, we have $\left\lfloor \frac{2n}{d} \right\rfloor \geq d^2 - d + 2$, making the linear bound dominant.
\end{proof}

The bound $|C| \leq \left\lfloor \frac{2n}{d} \right\rfloor$ is tight for large $n$, as shown by the optimal $\Delta(n, d/2, 0)$-system construction.

\begin{question}
    For a binary simplex code $C \subseteq H_2^n$ with distance $d$ to satisfy
    \[
    |C| \leq \frac{2n}{d},
    \]
    what is the best lower bound on $n$? Can the condition $n \geq O(d^3)$ be improved to $n \geq O(d^2)$ or $n \geq O(d)$?
\end{question}

\section{Discussions}
\label{section_discussion}

By Theorem \ref{theorem_upper_bound_with_d_binary_case}, for any binary simplex code \( C \subseteq H_2^n \) with even distance \( d \), if \( n \geq \frac{d(d^2 - d + 2)}{2} \), then the size of the code is bounded by
\[
|C| \leq \left\lfloor \frac{2n}{d} \right\rfloor.
\]

Let \( f(d) \) represent the smallest integer such that any binary simplex code of length \( n \geq f(d) \) satisfies this bound. From the proposition, we derive the estimate
\[
f(d) \leq \frac{d(d^2 - d + 2)}{2}.
\]

Here, we focus on determining \( f(d) \) for \( d = 4 \). Substituting \( d = 4 \) into the inequality, we obtain \( f(4) \leq 28 \). However, Example \ref{example_simplex_code_maximum_size} provides a binary simplex code \( C \subseteq H_2^7 \) with distance \( d = 4 \) and cardinality \( |C| = 8 \). For this code, since \( \frac{2n}{d} = \frac{n}{2} \), we compute \( \frac{2 \cdot 7}{4} = \frac{7}{2} = 3.5 \), and \( \left\lfloor 3.5 \right\rfloor = 3 \), which is less than 8. Thus, the bound \( |C| \leq \left\lfloor \frac{n}{2} \right\rfloor \) does not hold for \( n = 7 \). The bound becomes effective at \( n = 16 \), matching the cardinality of the example code. This implies:
\[
16 \leq f(4) \leq 28.
\]

This interval could be tightened by relaxing the cardinality constraints for an \( (n, k, l) \)-family to form a \( \Delta \)-system in Deza’s theorem. Furthermore, experimental programming results indicate that the maximum size of a binary simplex code remains \( 8 \) for \( 7 \leq n \leq 12 \), suggesting that \( f(4) \) may be closer to 16 than to 28.


\section{Discussions}
\label{section_discussions}

In this section, we propose several open questions for further explorations.

\begin{question}
Are there other equidistant codes $C \subseteq H_q^n$ that attain the upper bound $(q-1)n + 1$, except those presented in Example \ref{example_equidistant_code_maximum_size}?
\end{question}

\begin{question}
Denote $f_q(k,l)$ the smallest integer $m$ such that any $(n,k,l)_q$-family of cardinality greater than $m$ forms a $\Delta_q(n,k,l)$-system. By Theorem~\ref{theorem_q_ary_version_of_Deza_theorem}, we know 
\[f_q(k,l)\le  4(k - l)^2 + 2(k - l) + 1,\]
when $\max\{2l + 2, q - 1\}\le  4(k - l)^2 + 2(k - l) + 1$. What is the exact value of $f_q(k,l)$?
\end{question}

\begin{question}
For an equidistant code $C \subseteq H_q^n$ with distance $d$ satisfying
\[
|C| \leq \frac{2n}{d},
\]
what is the exact lower bound on $n$? 
\end{question}

We denote $f_q(d)$ the smallest integer $n_0$ such that whenever $n\ge n_0$ the inequality $|C|\le \frac{2n}{d}$ holds for any equidistant code $C\subseteq H_q^n$ with distance $d$. Then Corollary~\ref{corollary_bound_for_q_ary_equidistant_code} tells us that, viewing $q$ as a constant, $f_q(d)$ is at most $O(d^3)$. 

In fact, $f_q(d)$ lies in the interval $[\frac{d(d^2+2d+4)}{8},\frac{d(d^2+d+2)}{2}]$ when $d/2$ is a prime power and $q\le d^2+d+2$. Consider projective plane $PG(2,k)$, where $k$ is an prime power. Note that $PG(2,q)$ is an $(k^2+k+1,k+1,1)$-family and also a $q$-ary equidistant code of length $n = k^2+k+1$, distance $ d = 2k$ and size $k^2+k+1$. Let $C\subseteq H_q^{n_0}$ be an equidistant code of maximum size with distance $d$, where $n_0=f_q(d)$. Then we have 
\[k^2+k+1 = \frac{d^2}{4}+\frac{d}{2}+1\le |C|\le \frac{2f_q(d)}{d}.\]
Therefore,
\[f_q(d)\ge \frac{d(d^2+2d+4)}{8}.\]
On the other hand, by Corollary \ref{corollary_bound_for_q_ary_equidistant_code}, we have 
\[f_q(d)\le \frac{d(d^2+d+2)}{2},\]
when $q\le d^2+d+2$. 

Note that by Corollary~\ref{corollary_distant_dependent_bound_binary_case}, for binary case, we have
\[f_2(d)\le \frac{d(d^2+2d+8)}{8}.\]
Therefore, we conclude that $f_2(d)$ lies in the interval $[\frac{d(d^2+2d+4)}{8},\frac{d(d^2+2d+8)}{8}]$ when $d/2$ is a prime power.



==> settings.tex <==
\usepackage{graphicx} 
\usepackage{amsmath}    
\usepackage{amssymb}    
\usepackage{amsthm}    
\usepackage{dsfont}
\usepackage[a4paper, left=1in, right=1in, top=1in, bottom=1in]{geometry} % Page size and margins
\usepackage{hyperref}
\usepackage{xcolor}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}


\theoremstyle{definition}
\newtheorem{conjecture}{Conjecture}
\newtheorem*{remark}{Remark}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{question}{Question}
\newtheorem{claim}{Claim}


